REL-SF4PASS: Panoramic Semantic Segmentation with REL Depth Representation and Spherical Fusion

As an important and challenging problem in computer vision, Panoramic Semantic Segmentation (PASS) aims to give complete scene perception based on an ultra-wide angle of view. Most PASS methods often focus on spherical geometry with RGB input or using the depth information in original or HHA format, which does not make full use of panoramic image geometry. To address these shortcomings, we propose REL-SF4PASS with our REL depth representation based on cylindrical coordinate and Spherical-dynamic Multi-Modal Fusion SMMF. REL is made up of Rectified Depth, Elevation-Gained Vertical Inclination Angle, and Lateral Orientation Angle, which fully represents 3D space in cylindrical coordinate style and the surface normal direction. SMMF aims to ensure the diversity of fusion for different panoramic image regions and reduce the breakage of cylinder side surface expansion in ERP projection, which uses different fusion strategies to match the different regions in panoramic images. Experimental results show that REL-SF4PASS considerably improves performance and robustness on popular benchmark, Stanford2D3D Panoramic datasets. It gains 2.35% average mIoU improvement on all 3 folds and reduces the performance variance by approximately 70% when facing 3D disturbance.

==> tables/Statics_SGAM_big.tex <==
\renewcommand{\arraystretch}{1.5}
\begin{table*}
    \footnotesize
    \centering
    \resizebox{0.95\textwidth}{!}{
        \begin{tabular}{c|c|c|c|c|c}
        \hline
        \multirow{2}{*}{($\beta$,$\gamma$,$\alpha$) ($^{\circ}$)} & HHA mIoU / PAcc   & \multirow{2}{*}{($\beta$,$\gamma$,$\alpha$) ($^{\circ}$)} & HHA mIoU / PAcc   & \multirow{2}{*}{($\beta$,$\gamma$,$\alpha$) ($^{\circ}$)} & HHA mIoU / PAcc   \\ 
        \cline{2-2} \cline{4-4} \cline{6-6}
                                                 & Our mIoU / PAcc &                                              & Our mIoU / PAcc &                                              & Our mIoU / PAcc \\ \hline
        \multirow{2}{*}{(0,5,0)}                     & 61.171 / 87.910         & \multirow{2}{*}{(5,0,0)}                     & 60.805 / 87.727         & \multirow{2}{*}{(5,5,0)}                     & 58.943 / 86.677         \\
        \cline{2-2} \cline{4-4} \cline{6-6}
                                                     & 64.337 / 89.411 &              & 64.031 / 89.293 &              & 62.730 / 88.693  \\ 
        \hline
        \multirow{2}{*}{(0,5,90)}                    & 61.017 / 87.671 & \multirow{2}{*}{(5,0,90)}                    & 61.638 / 88.182 & \multirow{2}{*}{(5,5,90)}                    & 59.030 / 86.418  \\ 
        \cline{2-2} \cline{4-4} \cline{6-6}
                                                     & 63.854 / 89.186 &               & 64.501 / 89.424 &               & 62.898 / 88.556 \\
        \hline
        \multirow{2}{*}{(0,5,180)}                   & 60.864 / 87.955 & \multirow{2}{*}{(5,0,180)}                   & 60.791 / 87.752 & \multirow{2}{*}{(5,5,180)}        & 58.816 / 86.889 \\
        \cline{2-2} \cline{4-4} \cline{6-6}
                                                     & 63.991 / 89.389  &             & 64.138 / 89.413  &              & 62.968 / 88.896 \\ 
        \hline
        \multirow{2}{*}{(0,5,270)}                   & 61.144 / 87.715 & \multirow{2}{*}{(5,0,270)}                   & 61.609 / 88.043 & \multirow{2}{*}{(5,5,270)}                   & 58.932 / 86.471 \\ 
        \cline{2-2} \cline{4-4} \cline{6-6}
                                                     & 64.257 / 89.398 &              & 64.215 / 89.404 &               & 62.551 / 88.498 \\
        \hline
        \end{tabular}
    }
    \caption{
    {\color{red}Detail performance comparison with CMX~\cite{zhang2023cmx} baseline with HHA input on Stanford2D3D Panoramic datasets official fold 1 with SGA metrics. }
    Detail situations are shown, and the analysis is in~\cref{tab:STA_SGAM_BIG}. 
    ``HHA'' means the CMX~\cite{zhang2023cmx} baseline. 
    ``PAcc'' meas the pixel accuracy metric. 
    }
    \label{tab:SGAMBIG}
\end{table*}


==> tables/ablationAH.tex <==
\begin{table}[]
    \footnotesize
    \centering
    \resizebox{0.42\textwidth}{!}{
    \begin{tabular}{c|cc}
    \hline
    Modal & mIoU   & Pixel accuracy \\
    \hline
    RGB         & 51.25 & 80.81      \\
    RGB-D       & 59.03 & 87.60      \\
    RGB-Angle   & 59.76 & 87.46      \\
    RGB-Height  & 62.47 & 89.96      \\
    RGB-EGVIA   & \textbf{63.35} & \textbf{88.78}      \\
    \hline
    \end{tabular}
    }
    \caption{Effect of each \ours module.  fold 1
    % We validate them on Stanford2D3D Panoramic datasets official fold 1 with traditional metrics.  
    % ``SGAIP'' / ``SDPE'' / ``PA'' means our SGA image projection / spherical deformable patch embedding / panorama-aware loss. 
    % Using anyone, an average improvement of 1.058\% mIoU / 0.365\% pixel accuracy is gained when using three gains 2.757\% / 1.652\%. 
    }
    \label{tab:ablationAH}
\end{table}

==> tables/ablationREL.tex <==
\begin{table}[]
    \footnotesize
    \centering
    \resizebox{0.42\textwidth}{!}{
    \begin{tabular}{c|cc}
    \hline
    Modal & mIoU   & Pixel accuracy \\
    \hline
    RGB         & 51.25 & 80.81      \\
    RGB-D       & 59.03 & 87.60      \\
    % RGB-HHA     & 63.98 & 90.04      \\
    RGB-ReD     & 62.02 & 88.97      \\
    RGB-EGVIA   & 63.35 & 88.78      \\
    RGB-LOA     & 61.28 & 88.45      \\  
    RGB-REL     & \textbf{64.47} & \textbf{89.49}      \\
    \hline
    \end{tabular}
    }
    \caption{Effect of each \ours module.  fold 1
    % We validate them on Stanford2D3D Panoramic datasets official fold 1 with traditional metrics.  
    % ``SGAIP'' / ``SDPE'' / ``PA'' means our SGA image projection / spherical deformable patch embedding / panorama-aware loss. 
    % Using anyone, an average improvement of 1.058\% mIoU / 0.365\% pixel accuracy is gained when using three gains 2.757\% / 1.652\%. 
    }
    \label{tab:ablationREL}
\end{table}

==> tables/perclass.tex <==
\begin{table*}[]
    \footnotesize
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|c|ccccccccccccc}
    \hline
    Modal     & mIoU  & beam & board & bookcase & ceiling & chair & clutter & column & door  & floor & sofa  & table & wall  & window \\ 
    \hline
    RGB-D     & 59.03 & 0.24 & 73.77 & 63.84 & 90.21 & 75.98 & 57.65 & 15.02 & 45.78 & 97.59 & 53.35 & 67.97 & 77.22 & 48.73 \\
    RGB-HHA   & 63.98 & 0.78 & 73.07 &	65.57 & 93.29 & 82.50 & 66.61 & 25.40 & 49.43 & 98.70 & 57.96 & 73.23 & 79.84 & 65.42 \\
    % RGB-REL   & 64.47 & 6.43 & 81.09 & 62.16 & 92.69 & 82.10 & 62.60 & 25.87 & 51.23 & 98.70 & 60.15 & 72.76 & 79.92 & 62.45 \\
    Ours  & 66.73 & 4.45 & 78.77 & 69.71 & 93.80 & 83.56 & 66.45 & 28.22 & 53.31 & 98.70 & 74.90 & 74.93 & 80.82 & 59.91  \\
    % \hline
    % Trans4Pass+ & \multirow{2}{*}{SGA}  & 50.03 & 0.26 & 73.78 & 62.21    & 83.82   & 61.87 & 32.11   & 10.93  & 20.26 & 92.96 & 38.33 & 61.78 & 74.35 & 37.73  \\
    % Ours        &                               & 55.98 & 0.78 & 73.94 & 65.56    & 84.08   & 64.39 & \color{red}{40.96}   & \color{red}{18.31}  & \color{red}{\textbf{51.64}} & 92.98 & \color{red}{\textbf{56.53}} & 58.14 & 76.06 & \color{red}{44.42}  \\& \multirow{4}{*}{fold 1}
    \hline
    \end{tabular}
    }
    \caption{    
    Per-class mIoU results on Stanford2D3D Panoramic datasets according to the fold 1 data setting with traditional metric mIoU. 
    The results show that \ours gain the highest mIoU on lost classes and gain at most 16.94 \% improvement on the basis of RGB-HHA. 
    % No mark for the results of RGB-REL / RGB-REL-G that the gap between RGB-HHA and RGB-REL / RGB-REL-G less than 6\% (performance at the same level). 
    % Our results will be {\color{red}red} when Ours outperforms RGB-HHA more than 6\%. 
    % If Ours outperforms more than 10\%, our results will be {\color{red}\textbf{bold and red}}.
    % There is no semantic class that RGB-HHA outperforms Ours 6\% or more.
    }
    \label{tab:per_class_miou}
\end{table*}

==> tables/table1.tex <==
\begin{table}[ht]
\centering
\caption{消融实验：不同模态和模块对性能的影响}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{实验设置} & \textbf{mIoU (\%)} & \textbf{参数量 (M)} & \textbf{推理时延 (ms)} & \textbf{NDS (\(\sigma = 0.1\))} \\ 
\hline
RGB  & 56.3 & 121 & 45 & 0.63 \\ 
\hline
RGB-HHA  & 61.7 & 133 & 53 & 0.71 \\
\hline
RGB-HHA-Thermal  & 62.2 & 151 & 67 & 0.68 \\
\hline
RGB-HHA-LiDAR  & 62.1 & 148 & 64 & 0.69 \\
\hline
去除 CM-FRM-S  & 58.6 & 130 & 56 & 0.68 \\
\hline
仅使用 Early Fusion  & 58.7 & 128 & 55 & 0.67 \\
\hline
替换为普通 SDPE  & 57.4 & 125 & 54 & 0.66 \\
\hline
\end{tabular}
\end{table}
